Classification of the Extremely Low Frequency Magnetic Field Radiation Measurement from the Laptop Computers

The paper considers the level of the extremely low-frequency magnetic field, which is produced by laptop computers. The magnetic field, which is characterized by extremely low frequencies up to 300 Hz is measured due to its hazardous effects to the laptop user's health. The experiment consists of testing 13 different laptop computers in normal operation conditions. The measuring of the magnetic field is performed in the adjacent neighborhood of the laptop computers. The measured data are presented and then classified. The classification is performed by the K-Medians method in order to determine the critical positions of the laptop. At the end, the measured magnetic field values are compared with the critical values suggested by different safety standards. It is shown that some of the laptop computers emit a very strong magnetic field. Hence, they must be used with extreme caution.

==> refs.tex <==
\begin{thebibliography}{10}

\bibitem{[1]}
IARC. (2002). Monographs on the Evaluation of Carcinogenic Risks to Humans, Vol. 80, Non-Ionizing Radiation, Part 1: Static and Extremely Low-Frequency (ELF) Electric and Magnetic Fields, IARC Press, Lyon, France.

\bibitem{[2]}
National Radiological Protection Board (NRPB). (2001). ELF Electromagnetic Fields and the Risk of Cancer, Report of an Advisory Group on Non-ionizing Radiation (Doc NRPB 12), Chilton, UK.

\bibitem{[3]}
World Health Organization (WHO). (2010). Extremely Low Frequency Fields. Environmental Health Criteria Monograph No. 238.

\bibitem{[4]}
Bellieni C.V., Pinto I., Bogi A., Zoppetti N., Andreuccetti D., Buonocore G. (2012).  Exposure to Electromagnetic Fields from Laptop Use of "Laptop" Computers. Archives of the Environmental and Occupational Health, 67(1), 31-36.	 DOI:10.1080/19338244.2011.564232.

\bibitem{[5]}
Fernie, K. J., Reynolds, S. J. (2005). The effects of electromagnetic fields from power lines on avian reproductive biology and physiology: a review. Journal of Toxicology and Environmental Health. Part B, Critical Reviews, 8(2), 127-140. DOI: 10.1080/10937400590909022

\bibitem{[6]}
Bastuji-Garin, S. R., and Zittoun, R. (1990). Acute leukemia in workers exposed to electromagnetic fields. European Journal of Cancer, 26, 1119-1120.

\bibitem{[7]}
Harrington, J. M., McBride, D. I., Sorahan, T., Paddle, G. M., and van Tongeren, M. 1997. Occupational exposure to magnetic fields in relation to mortality from brain cancer among electricity generation and transmission workers. Occupational and Environmental Medicine, 54, 7-13.

\bibitem{[8]}
Johansen, C., and Olsen, J. (1998). Mortality from amyotrophic lateral sclerosis, other chronic disorders and electric shocks among utility workers. American Journal of Epidemiology, 148, 362-368.

\bibitem{[9]}
Verkasalo, P. K., Kaprio, J., Varjonen, J., Romanov, K., Heikkila, K., and Koskenvuo, M. (1997). Magnetic fields of transmission lines and depression. American Journal of Epidemiology,146, 1037-1045.

\bibitem{[10]}
Sobel, E., Dunn, M., Davanipour, Z., Qian, Z., and Chui, H. C. (1996). Elevated risk of Alzheimer's disease among workers with likely electromagnetic field exposure. Neurology, 47, 1477-1481.

\bibitem{[11]}
Calvente, I., Fernandez M. F., Villalba, J., Ilea, N. (2010). Exposure to electromagnetic fields and its relationship with childhood leukemia: A systematic review. Science of  Total Environment, 408(16), 3062-2069. DOI: 10.1016/j.scitotenv.2010.03.039.

\bibitem{[12]}
ICNIRP, International commision on non-ionizing radiation protection. (1998). Guidelines for limiting exposure to time varying electric, magnetic and electromagnetic fields. Health Physics, 74, 494-522. 

\bibitem{[13]}
Koppel, T., Tint, P. (2014). Reducing exposure to extremely low frequency electromagnetic fields from portable computers. Agronomy Research, 12(3), 863-874.

\bibitem{[14]}
Bradley, P. S., Mangasarian, O. L. and Street, W. N. (1997). Clustering via Concave Minimization.  Advances in Neural Information Processing Systems, 9, 368-374.

\bibitem{[15]}
MacQueen, J. (1967). Some methods for classification and analysis of multivariate observations. In Fifth Berkeley Symposium on Mathematical Statistics and Probability, 1, 281-297.

\bibitem{[16]}
Mathews, J., Nair, M.S., Jo, L. (2012). Improved BTC Algorithm for Gray Scale Images Using K-Means Quad Clustering. Neural Information Processing, 7666, 9-17. DOI: 10.1007/978-3-642-34478-7\_2.

\bibitem{[17]}
\cite{[17]}	Prasad, S., Kumar, P., Sinha, K.P. (2015). Grayscale to Color Map Transformation for Efficient Image Analysis on Low Processing Devices. Advances in Intelligent Systems and Computing, 320, 9-18. DOI: 10.1007/978-3-319-11218-3\_2.

\bibitem{[18]}
Wang, H., Song, M. (2011). Ckmeans.1d.dp: Optimal k-means Clustering in One Dimension by Dynamic Programming. The R Journal, 3(2), 29-33.

\bibitem{[19]}
Gong, Y., Liu L., Yang, M., Bourdev, L. (2014). Compressing Deep Convolutional Networks using Vector Quantization. arXiv preprint arXiv:1412.6115.

\bibitem{[20]}
Anderson, B., Gross, D., Musicant, D., Ritz, A., Smith, T., Steinberg, L. (2006). Adapting K-Medians to Generate Normalized Cluster Centers. In SIAM International Conference on Data Mining, 20-22 April 2006. Bethesda,  Maryland, 165-175.

\bibitem{[21]}
Brodic, D., Tasic V. (2014). Exposure of the Laptop Users to the Extremely Low-Frequency Electromagnetic Field. In International Scientific Conference (UNITECH), 21-22 November 2014. Gabrovo, Bulgaria, 59-64.

\bibitem{[22]}
TCO Certified Tablets 1.0, TCO Development AB, \url{http://tcodevelopment.com/files/2012/06/criteriadocument\_tablets\_v10\_2011-10-20\_tcodevelopment.pdf}.
 
\end{thebibliography}

